Almost Optimal Stochastic Weighted Matching With Few Queries

We consider the {\em stochastic matching} problem. An edge-weighted general (i.e., not necessarily bipartite) graph $G(V, E)$ is given in the input, where each edge in $E$ is {\em realized} independently with probability $p$; the realization is initially unknown, however, we are able to {\em query} the edges to determine whether they are realized. The goal is to query only a small number of edges to find a {\em realized matching} that is sufficiently close to the maximum matching among all realized edges. This problem has received a considerable attention during the past decade due to its numerous real-world applications in kidney-exchange, matchmaking services, online labor markets, and advertisements. Our main result is an {\em adaptive} algorithm that for any arbitrarily small $\epsilon > 0$, finds a $(1-\epsilon)$-approximation in expectation, by querying only $O(1)$ edges per vertex. We further show that our approach leads to a $(1/2-\epsilon)$-approximate {\em non-adaptive} algorithm that also queries only $O(1)$ edges per vertex. Prior to our work, no nontrivial approximation was known for weighted graphs using a constant per-vertex budget. The state-of-the-art adaptive (resp. non-adaptive) algorithm of Maehara and Yamaguchi [SODA 2018] achieves a $(1-\epsilon)$-approximation (resp. $(1/2-\epsilon)$-approximation) by querying up to $O(w\log{n})$ edges per vertex where $w$ denotes the maximum integer edge-weight. Our result is a substantial improvement over this bound and has an appealing message: No matter what the structure of the input graph is, one can get arbitrarily close to the optimum solution by querying only a constant number of edges per vertex. To obtain our results, we introduce novel properties of a generalization of {\em augmenting paths} to weighted matchings that may be of independent interest.

==> generalweighted.tex <==
\sbcomment{Some of the definitions that were defined above will be removed or I will mention that we restate to remain self-contained.}

Consider two arbitrary weighted matchings $M_L$ and $M_H$ with $w(M_L) \leq (1-\epsilon)w(M_H)$. In this section, we show that one can find a set of vertex disjoint short {\em augmenting components} (a generalization of augmenting paths to weighted graphs) for $M_L$ and $M_H$ such that each of these augmenting components has a size of at most $O(1/\epsilon)$ and the total {\em augmentation value} of all these components is at least $\Omega(\epsilon w(M_H))$. This lemma is not limited to our model of stochastic graphs and applies to any graph, and thus, we believe is of independent interest to other settings as well.

Let us denote by $\diff{A}{B} := (A \cup B) - (A \cap B)$ the symmetric difference of two sets $A$ and $B$.
	Consider the graph $D := M_L\Delta M_H$ of edges that appear in exactly one of $M_L$ and $M_H$. Since the degree of each vertex in $D$ is at most 2 (due to the fact that both $M_1$ and $M_2$ are matchings), $D$ is a collection of vertex disjoint paths and cycles. We start by defining alternating- and augmenting-components.
	
\begin{definition}
	We call any connected component of $M_L \Delta M_H$ an {\em alternating component}. For an alternating component $C$, define $L_C := C \cap M_L$ to be its edges in $M_L$ and define $H_C := C \cap M_H$ to be its edges in $M_H$. We call $L_C$ the {\em light} portion of component $C$ and call $H_C$ the {\em heavy} portion of $C$. We further define the value of a component $C$ to be $w(H_C) - w(L_C)$ and denote it by $\Delta_C$. We call an alternating component $C$ with $\Delta_C > 0$ an augmenting component.
\end{definition}

Note that alternating/augmenting components in weighted graphs can be either cycles or paths, hence we refer to them as {\em components} instead of paths which is more common for cardinality matching in unweighted graphs. We are now ready to formalize our lemma.

\begin{lemma}[Alternating components decomposition lemma]
	For any constant $\epsilon \in (0, 1)$ and for any two weighted matchings $M_L$ and $M_H$ with $w(M_L) \leq (1-\epsilon)w(M_H)$, one can find a subset $M'_H$ of $M_H$ such that: (1) All augmenting components in $M_L\Delta M'_H$ have at most $4/\epsilon$ edges; (2) $w(M'_H) \geq (1-\frac{\epsilon}{2})w(M_H)$.
\end{lemma}

\begin{proof}
	To prove the lemma we remove the edges of $M_H$ to reduce the size of alternating components to at most $4/\epsilon$ while also ensuring that the total weight of removed edges is at most $\frac{\epsilon}{2} w(M_H)$. 
	
	Take an alternating component $C$ in $M_H \Delta M_L$ and suppose $C$ has more than $4/\epsilon$ edges. Depending on the structure of component $C$, denote its edges in the following way:
	\begin{enumerate}
		\item If $C$ is a path starting with an edge of $M_H$, denote its edges by $(h_1, l_1, h_2, l_2, \ldots)$ that is in the order that the edges appear in the path.
		\item if $C$ is a path starting with an edge of $M_L$, denote its edges by $(l_0, h_1, l_1, h_2, l_2, \ldots)$ that is in the order that the edges appear in the path.
		\item if $C$ is a cycle, denote its edges by $(h_1, l_1, h_2, l_2, \ldots)$ that is in the order that the edges appear in the cycle, starting from an arbitrary edge of $C$ that is part of matching $M_H$.
	\end{enumerate}
	Suppose for ease of exposition that $2/\epsilon$ is an integer. For any integer $i \in [1, 2/\epsilon]$, define $D_i$ to be the following set of edges of $M_H$ in $C$:
	\begin{equation*}
		D_i := \{ h_i, h_{i+ 2/\epsilon}, h_{i+4/\epsilon}, h_{i+6/\epsilon}, \ldots\}.
	\end{equation*}
	
	\begin{claim}\label{claim:shiftingsubsets}
		There exists some $i \in [1, 2/\epsilon]$ for which $w(D_i) \leq \epsilon w(H_C)/2$.
	\end{claim}
	\begin{proof}
		It is easy to confirm by definition that for any $i, j \in [1, 2/\epsilon]$ with $i \not= j$, we have $D_i \cap D_j = \emptyset$ and that $\cup_{i\in[1, 2/\epsilon)}D_i = H_C$. This means that $H_C$ is partitioned by $D_i$'s into $2/\epsilon$ disjoint subsets. Thus, the average total weight of $D_i$ for all $i \in [1, 2/\epsilon]$ is $\frac{w(H_C)}{2/\epsilon}$, meaning that there should be some $i \in [1, 2/\epsilon]$ with $w(D_i)$ no more than this average value.
	\end{proof}
	
	Now take an arbitrary $i \in [1, 2/\epsilon]$ for which $w(D_i) \leq \epsilon w(H_C)/2$ and delete all the edges of $D_i$ from $M_H$. Our claim is that if we do the same procedure for all augmenting components in $M_H\Delta M_L$ we obtain our desired graph $M'_H$. 
	
	One can confirm that this edge removal procedure decomposes each component $C$ into subcomponents of size at most $4/\epsilon$ since the gap between the consecutive indices of the edges in $D_i$ is $2/\epsilon$ (the extra factor of $2$ in $4/\epsilon$ is due to the edges of $L_C$ that appear in the component).
	
	It remains to prove that $w(M'_H) - w(M_L) \geq \frac{\epsilon}{2}w(M_H)$. To show this, observe that by Claim~\ref{claim:shiftingsubsets}, from each component $C$ we remove a weight of at most $\epsilon w(H_C)/2$. Therefore, we have the following bound on the weight of $M'_H$:
	\begin{flalign*}
		w(M'_H) &\geq w(M_H) - \sum_{C \in M_H\Delta M_L} \epsilon w(H_C)/2\\
		&\geq w(M_H) - \frac{\epsilon}{2} \sum_{C \in M_H\Delta M_L} w(H_C)\\
		& \geq w(M_H) - \frac{\epsilon}{2} w(M_H)\\
		& = (1-\frac{\epsilon}{2})w(M_H)
	\end{flalign*}
	which is the desired bound on the size of $M'_H$ concluding the lemma.
\end{proof}




